Learning Representations that Support Robust Transfer of Predictors

Ensuring generalization to unseen environments remains a challenge. Domain shift can lead to substantially degraded performance unless shifts are well-exercised within the available training environments. We introduce a simple robust estimation criterion -- transfer risk -- that is specifically geared towards optimizing transfer to new environments. Effectively, the criterion amounts to finding a representation that minimizes the risk of applying any optimal predictor trained on one environment to another. The transfer risk essentially decomposes into two terms, a direct transfer term and a weighted gradient-matching term arising from the optimality of per-environment predictors. Although inspired by IRM, we show that transfer risk serves as a better out-of-distribution generalization criterion, both theoretically and empirically. We further demonstrate the impact of optimizing such transfer risk on two controlled settings, each representing a different pattern of environment shift, as well as on two real-world datasets. Experimentally, the approach outperforms baselines across various out-of-distribution generalization tasks. Code is available at \url{https://github.com/Newbeeer/TRM}.

==> analysis.tex <==
To help us build insights into the optimal features for different methods, we first focus on an illustrative 2-d example with linear $\Phi$. We take inspiration from \cite{Rosenfeld2020TheRO} to construct  invariant $z_c$ and non-causal features $z_e$ by label-conditioned Gaussians. We consider linear feature extractor $\Phi(x)=az_c+bz_e$. To characterize algorithm behavior, we define spurious-to-invariant ratio of estimated weights $r_{alg}= |\frac{\argmin_b \gR_{alg}}{\argmin_a \gR_{alg}}|,  alg\in\{\textrm{ERM,IRMv1,TRM}\}$. $r_{alg}$ is the absolute value of the ratio between optimal weights associated with non-causal features and invariant features. Smaller weight ratio implies better performance on unseen environments, \ie the model places larger emphasis on invariant features. 

In this section, we show that all the methods can achieve zero weight ratio in an unbiased setting~(Proposition~\ref{prop:irmtrm}).  Observation~\ref{obs:weight-ratio} further shows that TRM generally yields smaller (approximate) weight ratio when training environments are biased. The theoretical results coincide with our experiments in Sec~\ref{exp:synthetic}, where all methods perform well without confounding non-causal features, and TRM outperforms others when non-causal features are present. 

\subsection{Data generation process}
\label{sec:data-gen}
For each environment, the data are defined by the following process: the binary label $y$ is sampled uniformly from $\{\pm 1\}$ and the input data $x=[z_c,z_e]$ are sampled subsequently from label-conditioned Gaussians:
\[z_c \sim \gN(y*\mu_c,1) ; z_e \sim \gN(y*\mu_i,1),i \in \{1,\dots,E\}\]
The invariant feature mean $\mu_c$ remains the same for all environments while non-causal means $\mu_i$s vary across environments. We denote the mean and variance of non-causal means as $\E_i \mu_i = {\sum_{i=1}^E \mu_i}/{E}$ and $\textrm{Var}(\mu_i)= \sum_{i=1}^E (\mu_i - \E_i \mu_i)^2/E$. We call the training environments unbiased when $\E_i \mu_i=0$ and biased otherwise.

\subsection{Comparison in linear case}
\label{exp:linear-case}
We adopt the logistic loss $\ell (x)=\log{(1+e^{-x})}$ and analyze the weight ratios in the population setting (unlimited samples from each environment). Our goal is to characterize the associated weight ratios for TRM, IRMv1 and ERM as a proxy measure for their ability to generalize to out-of-distribution settings. 
For simplicity, we use the ``sum-sum" version of TRM, \ie 
$\E_{i\not=j}\E_{(x,y)\sim P_j}\left[\ell(y\Phi(x)w(P_i))\right]$.
% \Eqref{eq:symmetry} holds by the symmetry of $\Phi(x)$ given $y=\pm 1$. Substituting the expression of $w(P_i)$ and $\Phi(x)$ into \Eqref{eq:symmetry}, we have:
% \begin{align*}
%     \gR_{TRM}(\Phi)=&\E_{i\not =j,z_c ,z_e,y}\left[f(2y\frac{(az_c+bz_e)(a\mu_c+b\mu_i)}{a^2 +b^2})\right]\numberthis \label{eq:logistic-loss}
% \end{align*}
The optimal values of weights for objectives are scale-invariant to $a^2+b^2$, hence w.l.o.g we assume $a^2+b^2=1$ in the following. To start with, we show that different objectives will learn robust linear feature extractors when $\E_{i}[\mu_i]=0$.
\begin{restatable}{proposition}{prefect}
\label{prop:stationary}
When $\E_{i}[\mu_i]=0$, the optimal weights ratios $r_{alg}=0,alg\in\{\textrm{ERM,IRMv1,TRM}\}$. 
\end{restatable}
The proposition shows that all the objectives are robust in the unbiased setting ($\E_{i}[\mu_i]=0$) in the sense that the resulting models use \textit{only} invariant features for the prediction. However, this does not hold when the training environments are biased, \ie, $\E_{i}[\mu_i]\not = 0$. By symmetry, we only consider $\E_{i}[\mu_i] > 0$. Since the optimal weight ratios under the biased setting have no analytic form, we introduce approximate values
$\hat{r}_{alg},alg\in\{\textrm{ERM,IRMv1,TRM}\}$. We defer the associated expressions and their tightness to Appendix~\ref{app:approx}. 
We show that TRM encourages the approximated weight ratio to be smaller than those for ERM and IRMv1 under mild conditions. We denote the average square loss for the optimal IRMv1 model as $k=\E_{i,x,y}(\frac{1}{1+\exp{(-w\circ \Phi(x))}}-\mathbb{I}(y=1))^2$, and the regularization coefficient in IRMv1 as $\lambda$. We have the following observation:

\begin{restatable}{observation}{weight}
\label{obs:weight-ratio}
Suppose $\textrm{Var}(\mu_i)>0$ and $\forall i, \mu_c \ge \mu_i, \mu_c \ge 1$, the approximated optimal weight ratios for ERM, IRMv1 and TRM satisfy $\hat{r}_{ERM}\ge \hat{r}_{IRMv1}, \hat{r}_{ERM}\ge \hat{r}_{TRM}$. If $k \le \frac{2}{\lambda E}$, then we have:
\begin{enumerate}[(i)]
    \item $\hat{r}_{ERM} > \hat{r}_{IRMv1} > \hat{r}_{TRM}$
    \item $\hat{r}_{ERM}/\hat{r}_{TRM}, \hat{r}_{IRMv1}/\hat{r}_{TRM}$ both decrease with the invariant feature mean $\mu_c$ and the number of environments $E$.
    \item $\hat{r}_{ERM}/\hat{r}_{IRMv1}$ increases with $k$. When $k=0$, $\hat{r}_{ERM}=\hat{r}_{IRMv1}$
\end{enumerate}
\end{restatable}

% We have following approximations for the relative magnitude of weights ratios when $\mu_c \ge \mu_i\ge 0.5, i\in \{1,\dots,E\}$:
% \begin{align*}
% \frac{r_{ERM}}{r_{TRM}}&\approx\frac{\mu_c^2 - C_T+\sqrt{(\mu_c^2 - C_T)^2+4(\mu_c\E{\mu_i})^2}}{\mu_c^2 - C_E+\sqrt{(\mu_c^2 - C_E)^2+4(\mu_c\E{\mu_i})^2}}\\
% \frac{r_{IRMv1}}{r_{TRM}}&\approx\frac{\mu_c^2 - C_T+\sqrt{(\mu_c^2 - C_T)^2+4(\mu_c\E{\mu_i})^2}}{\mu_c^2 - C_I+\sqrt{(\mu_c^2 - C_I)^2+4(\mu_c\E{\mu_i})^2}}z    
% \end{align*}



Observations~\ref{obs:weight-ratio}(i) shows that TRM learns better model with smaller optimal weight ratio. Note that the condition $k\le \frac{2}{\lambda E}$ generally holds since the linear model can easily fit the IRMv1 objective. The margin of TRM over other methods decreases with increasing $\mu_c$ and $E$. The result coincides with the intuition that ERM/IRMv1 would better recover $z_c$ when $z_c$ is easier for classification~(larger $\mu_c$), or adding more environments~(larger $E$). (iii) indicates that the advantage of IRMv1 over ERM vanishes when the model overfits the training set~(small $k$), as observed in \cite{Gulrajani2020InSO, Rosenfeld2020TheRO}. We defer all detailed analysis in this section to Appendix~\ref{app:proofs}. 

\begin{figure*}[t]
    \centering
   \subfigure[Varying $\mu_c$ with $E=5$]{\includegraphics[width=0.28\linewidth]{img/syn_swap.pdf}\label{img:muc}}% \hi
   \subfigure[Varying $E$ with $\mu_c=1$]{\includegraphics[width=0.28\linewidth]{img/syn_swap_envs.pdf}\label{img:E}}%
   \subfigure[Distance versus iteration]{\includegraphics[width=0.28\linewidth]{img/l2_dist.pdf}\label{fig:l2}}
    \caption{(a,b): Comparisons of the weights ratios; (c): Average square distance between per-environment predictors during training when $\mu_c=1,E=5$.}
    \label{img:analysis}
    \vspace{-3pt}
\end{figure*}
In addition to the theoretical analysis, we provide further empirical results for the optimal weight ratios. We synthesize the dataset by the data generation process in \Secref{sec:data-gen}, and use Adam with a learning rate $0.01$ as the optimizer. We set the expected non-causal mean $\E_i \mu_i$ and variance $\textrm{Var}(\mu_i)$ to 1. We randomly sample 10000 datapoints for each environment. We conduct experiments by varying $\mu_c$ and $E$. We defer more training details to Appendix~\ref{app:toy}.

\Figref{img:analysis}(a,b) report the theoretical approximations~( $\frac{\hat{r}_{ERM}}{\hat{r}_{TRM}},\frac{\hat{r}_{IRMv1}}{\hat{r}_{TRM}}$) and their practical values~( $\frac{r_{ERM}}{r_{TRM}},\frac{r_{IRMv1}}{r_{TRM}}$). The empirical values align well with the approximations with larger $\mu_c$ and $E$. We observe that TRM is more robust under various $\mu_c$s and $E$s, and its margin vanishes as $\mu_c$ and $E$ increase. In \Figref{fig:l2}, we visualize the average square distance between per-environment predictors in TRM. The distance between different environmental predictors gradually converges to some small value. The results suggests that TRM better drives the representation toward invariance across environments during training.


==> dump.tex <==
% \section{Self-invariant learning}

% \subsection{Setup}

% Most (unsupervised) pretrained networks are often highly redundant and captures both the spurious correlation and the invariant relationship between input and its label. We want to pursuit invariant representation on such large pretrained networks. In our experiment in \secref{exp}, we show that the pretrained network can both capture the information of invariant and spurious features. In the light of this, we want to further avoid using the spurious features.

% We have a set of sub-networks $\{g_{\theta_1}, \dots, g_{\theta_n}\}$ of the pretrained networks, classifier $f$ and loss function $\Ls$. And we make the following assumptions:

% \textbf{Assumptions:}
% \begin{enumerate}
%     \item Classifiers $f$ training on the top of all the sub-networks have small training loss. 
%     \item These sub-networks are diverse w.r.t the spurious features.
%     \item These sub-networks make predictions mainly on the information of invariant features.
% \end{enumerate}

% Assumption 1 requires all of the sub-networks learn the discriminative things out of the spurious/invariant features. Assumption 2\&3 enable us to find the common-ground feature ( the invariant feature) out of these sub-networks. 

% % To make the inductive bias of sub-networks more consistent with assumptions above, we can explicitly enforce $\{g_{\theta_1}, \dots, g_{\theta_n}\}$ to share some common channels $\gC$ in the last layer, and $g_{\theta_i}=\gC \cup {\gC_i}$. \yx{implicitly define an order on channels?}
% % We define a discrepancy measure $D$ on the function space. The direct objective is 
% % \[i,j = \max\limits_{i,j} D(g_{\theta_i},g_{\theta_j})\]

% % We have two classifiers on $g_{\theta_i},g_{\theta_j}$ respectively, 

% % \[f_i = \argmin \Ls(f_i \circ g_{\theta_i}), f_j = \argmin \Ls(f_j \circ g_{\theta_j})\]

% In the following we denote each sub-networks as $SN_i = f_i \circ e \circ g_i$, where $e$ is a shared backbone.

% We define the regret of sub-network $i$ as:\[R(SN_i) =\E_{j \sim \sU[1,n]}\left[\Ls(f_j \circ e \circ g_{\i})\right]\]
% where $f_j = \argmin \Ls(f_j \circ e \circ g_{j})$, and $\sU[1,n]$ denotes a uniform distribution over $\{1,2,\cdots,n\}$.

% % We formulate the self-invariant learning as a mini-max setting. We firstly select the pair of sub-networks that maximize the discrepancy, i.e. the regret. Then we minimize the maximal regret.
% % \[\min\limits_{g_{1}, \dots, g_{n}}\max\limits_{i,j} R(SN_i, SN_j) \numberthis \label{loss:robust}\]
% \subsection{Analysis \yx{sloppy}}

% Assume the output of a specific layer $k$ as $h_k \in \R^d$. We sample a scaling vector $\eta\in \R^d$ with independent random coordinates
% \[ \eta_i =\left\{
% \begin{aligned}
% &-1 \quad \textrm{with probability } q \\
% &\frac{q}{1-q} \quad \textrm{with probability } 1-q \\
% \end{aligned}
% \right.\]

% For two sub-networks $g_1,g_2$, denote the output at layer $k$ as $h_k^1,h_k^2 \in \R^d$. Then we have $h_k^1=h_k^2+(\eta^1-\eta^2)\odot h_k$. Apparently we have $\eta^i \odot h_k$ as zero mean vector. Denote $\delta = (\eta^1-\eta^2)\odot h_k$. Note that $\delta$ is zero mean vector as well.

% Take the Taylor expansion we have 
% \begin{align*}
%     \Ls(f_2 \circ h_k^1) - \Ls(f_2 \circ h_k^2) \approx D_{h_k^2}(\Ls(f_2 \circ h_k^2))\delta + \delta^T D_{h_k^2}^2\Ls(f_2 \circ h_k^2))\delta
% \end{align*}
% Take expectation on both sides (assume infinite sub-networks) we get
% \begin{align*}
%     \E_{\delta}\left[\Ls(f_2 \circ h_k^1) - \Ls(f_2 \circ h_k^2)\right] & \approx \underbrace{\E_{\delta}D_{h_k^2}(\Ls(f_2 \circ h_k^2))\delta}_{0}+\E_{\delta}\left[\delta^T D_{h_k^2}^2\Ls(f_2 \circ h_k^2))\delta\right]\\
%     &=\langle D_{h_k^2}^2\Ls(f_2 \circ h_k^2),\E_{\delta} \left[\delta^T\delta\right]\rangle\\
%     &=\frac{2q}{1-q} \langle D_{h_k^2}^2\Ls(f_2 \circ h_k^2),diag(h_k \odot h_k)\rangle \\
%     &=\langle J_{h_k^2}(f_2 \circ h_k^2)^T D_{f_2}^2(\Ls(f_2 \circ h_k^2))J_{h_k^2}(f_2 \circ h_k^2) + \underbrace{ \sum_i (D_{f_2}\Ls(f_2 \circ h_k^2))_i D_{h_k^2}^2((f_2 \circ h_k^2)_i)}_{\approx 0},diag(h_k \odot h_k)\rangle\\
%     &=\langle J_{h_k^2}(f_2 \circ h_k^2)^T D_{f_2}^2(\Ls(f_2 \circ h_k^2))J_{h_k^2}(f_2 \circ h_k^2),diag(h_k \odot h_k)\rangle
% \end{align*}

% The major difference between self-invariant learning (with infinite sub-networks) and Dropout is we can get rid of the non-PSD term $ \sum_i (D_{f_2}\Ls(f_2 \circ h_k^2))_i D_{h_k^2}^2((f_2 \circ h_k^2)_i)$.

% Denote $h_k^+ =h_k + \eta\odot h_k$, and $f^+ = \argmin \Ls(f \circ h_k^+)$, then the expectation of regularization is:
% \begin{align*}
%     \E_{\eta}[\langle J_{h_k^+}(f^+ \circ h_k^+)^T D_{f^+}^2(\Ls(f^+ \circ h_k^+))J_{h_k^+}(f^+ \circ h_k^+),diag(h_k \odot h_k)\rangle] \numberthis
% \end{align*}

% Consider the norm of the gradient $\parallel J_{h_k^+}(f^+ \circ h_k^+) \parallel_2$,
% \begin{align*}
%     \E_{\eta}\parallel J_{h_k^+}(f^+ \circ h_k^+) \parallel_2^2 &= \E_{\eta} \parallel J_{h_k}(f^+ \circ h_k^+) \parallel_2^2 \\
%     &\approx \E_{\eta}[\parallel J_{h_k}(f^+ \circ h_k)+  D_{h_k}^2(f^+ \circ h_k)\eta \parallel_2^2]\qquad\textrm{(Taylor expansion)}\\
%     &= \E_{\eta}\parallel J_{h_k}(f^+ \circ h_k) \parallel_2^2 + \E_{\eta}[\parallel D_{h_k}^2(f^+ \circ h_k)\eta \parallel_2^2]\\
%     &\approx\E_{\eta}\parallel J_{h_k}(f^+ \circ h_k) \parallel_2^2 + C* (Tr(D_{h_k}^2(f^+ \circ h_k)))^2 \qquad\textrm{(Hutchinson trace estimator)}\numberthis\\
% \end{align*}

% \subsection{Implementation}


% % \begin{proposition}
% % There exists $\lambda_{i,j}>0$ such that the minimizer in loss (\ref{loss:robust}) is the first order stationary point of $\sum\limits_{i,j} \lambda_{i,j} R(SN_i, SN_j)$. 
% % \end{proposition}


% \paragraph{Loss function}In practice we select $\lambda_{i,j}=1$. Combining with the prediction loss, we use the following loss for the self-invariant learning:
% \[\sum\limits_{i} \Ls(SN_i) + \lambda \sum\limits_{i} R(SN_i)\numberthis\]

% \paragraph{Architecture for sub-networks}
% We carefully design the architecture for sub-networks in order to induce the diversity. For each sub-network, we randomly selects a set of neurons and removes (or say masking) them from the network before training. To apply masking on a selected layer $Layer(j)$, suppose the input is $X_j$ and the output is $conv_j(X_j) \in \mathbb{R}^{m_j\times n_j\times c_j}$. We randomly generate a binary mask $mask(j) \in \{0,1\}^{m_j\times n_j\times c_j}$ by sampling uniformly within each channel with drop-out ratio $r$. Then we mask the neurons in position $(x, y, c)$ of the output of $Layer(j)$ if the $(x, y, c)$ element of $mask(j)$ is zero. We sample the mask independently for each sub-network .

% \paragraph{Experiment on PACS dataset} We follow the setup in the paper \cite{Gulrajani2020InSO}. We use three sub-networks in self-invariant learning and set the drop-out ratio to $0.1$.
% \begin{table}[htp]
% \caption{Test accuracy on PACS dataset}
% \label{table:clothing1M}
% \begin{center}
% \begin{tabular}{c c c c c c c c}
% 		\toprule
% 		\textbf{Algorithm} & \textbf{Art} & \textbf{Cartoon} & \textbf{Photo} & \textbf{Sketch}	& \textbf{Average}\\
% 		\midrule
%         ERM & $87.3$ & $81.8$ & $95.5$ & $81.3$ & $86.5$ \\
%         \midrule
%         Self-invariant & $88.26$ & $83.5$ & $94.0$ & $82.9$ & \textbf{87.2} \\
% 		\bottomrule
% \end{tabular}
% \end{center}
% \end{table}

% \subsection{Theoretical insights}
% We can develop some theoretical arguments to show that once $\{g_{\theta_1}, \dots, g_{\theta_n}\}$ achieves mini-max optimal, their representations are biased toward the invariant features.

% Consider the linear case where $g_{\theta_i}(x)=(w_i^1,w_i^2)^T\vx$. Classifiers $f$ is an threshold function. $x_1$ is the invariant feature while $x_2$ is the spurious feature. To meet assumption 2, we need to assume that the weights $w_i^2$ can only change slightly during the optimization process \yx{unrealistic?}. We can show that during the optimization process of the mini-max game the norm of $w_i^1$ increase largely.

\section{Optimality of IRM}

(The generation process is taken from paper  \hyperlink{https://openreview.net/forum?id=BbNIbVPJ-42}{'The risks of invariant risk minimization'})\\
There are $E$ training environments $\{e_i\}_{i=1}^E$. For a given environment $e$, the data generating process is :
\begin{align*}
    y=\left\{
\begin{aligned}
&1 \quad \textrm{w.p.} \quad p \\
&-1 \quad \textrm{otherwise}
\end{aligned}
\right.
\end{align*}

Next, the invariant features and the environmental features for $e$ are drawn according to Gaussians:

$$z_c \sim \gN(y\mu_c, \sigma_c^2I),z_e \sim \gN(y\mu_e, \sigma_e^2I)$$
with $\mu_c \in \sR^{d_c},\mu_e \in \sR^{d_e}$. Finnaly the observation $x$ is generated as a function of the latent features:

$$x=f(z_c,z_e)$$
We assume $f$ is injective, so that it is in principle possible to recover the latent features $z_c,z_e$ from the observations. The objective is to learn a feature embedder $\Phi$ and a regression vector $\beta$ to minimize the risk on an unseen enviroment $e$:
\begin{align*}
    R^e(\Phi, \beta)=\E_{x,y}[\Ls(\sigma(\beta^T\Phi(x)),y)]
\end{align*}

where $\sigma$ is the sigmoid function. Apparently the invariant classifier comprise:
$\Phi(x)=\begin{bmatrix}I&0\\0&0\end{bmatrix}f^{-1}(x)=\begin{bmatrix}z_c & 0\end{bmatrix}, \beta = \begin{bmatrix}2\mu_c/\sigma_c & 0\end{bmatrix}$

Assume $f$ is linear. The paper \hyperlink{https://openreview.net/forum?id=BbNIbVPJ-42}{'The risks of invariant risk minimization'} told us that if $E\le d_e$ and the environmental means $\mu_e$ are linear independent, then there exists a linear $\Phi$ whose output depends on the environmental features, yet the optimal classifiers $\beta$ on the top of $\Phi$ is invariant across environments. Also, under some mild conditions it achieves lower risk than the invariant classifiers.
\begin{theorem}
Suppose $E\le d_e$. If there exists an environments $\hat{e}$ such that $\mu_{\hat{e}} = \sum_{e_i\not = \hat{e}} \alpha_i \mu_{e_i}$, and $\sum_{e_i\not = \hat{e}} \alpha_i\not =1, \sum_{e_i\not = \hat{e}} \alpha_i\sigma_i=\sigma_{\hat{e}}$. Let $\Phi(z_c,z_e)=Az_c+Bz_e$, then linear featurerizer $\Phi$ with an invariant optimal regression vector $\beta$ must satisfies $B\mu_e = 0,\forall e \in \gE$.
\end{theorem}

We can expect that if a test environment whose environmental feature mean lies in the $Span\{\mu_e, e\in \gE\}$, the $(\Phi,\beta)$ pair would not fail.

It also implies that we can construct an extra environment, which does not lie in the convex hull of the other environments, to test whether the optimal regression vector $\beta$ uses only the invariant features.

















\section{Ordered neurons}

Suppose we have a set of neurons $\{\theta_1,\dots,\theta_n\}$ in a large neural network $\Theta$. We would like to impose an order on the set of neurons. We introduce the following nested loss:

\[\Ls = \E_{(x,y)\sim p(x,y)}\E_{i\sim \sU[1,n]}\Ls(f_{\theta_1,\dots,\theta_i}(x),y) \label{loss:order} \numberthis\]

When we use neuron $\theta_i$, neuron $\theta_1,\dots,\theta_{i-1}$ also need to be taken in computation. Apparently, the importance of the $i$-th network decrease with its index. Thus we can adapt network capacity to the real-time computational budges. We can build a single model that can automatically trade-off computational cost versus accuracy.

\subsection{Theoretical insights}

\subsubsection{Natural ordering} 

\begin{theorem}
    Let $(x,y) \sim p_d(x,y)$. And we denote $q_{\theta_1,\dots,\theta_i}(z|x)$ as $q_{\theta}(z_{\le i}|x)$ for simplicity. Assume $z_i \perp z_{i+1} | y,z_{i\le 2}$. Then we can derive the conditional mutual information decrease w.r.t $i$ when the neurons are optimal in terms of minimizing the cross-entropy loss. Informally, we have \[I(z_i;y|z_{ \le i-1}) \le I(z_{i-1};y|z_{ \le i-2})\]
\end{theorem}
    
proof: refer to appendix.


In practice, the conditional mutual information can be express as the decreasing amount of accuracy, as shown in \figref{img:img-dimension}(b). 
\begin{figure*}[htbp]
    \centering
  \subfigure[Top-1 accuracy under different model sizes ]{\includegraphics[width=0.5\linewidth]{img/acc_parameters.pdf}}%
  \subfigure[Top-1 accuracy under different FLOPS]{\includegraphics[width=0.5\linewidth]{img/acc_flops.pdf}}
  \caption{The Top-1 accuracy of ResNet34 models on the ImageNet dataset.}
    \label{img:img-dimension}
\end{figure*}
\begin{figure*}[htbp]
    \centering
  \subfigure[Accuracy under different model sizes ]{\includegraphics[width=0.5\linewidth]{img/bert_acc_parameters.pdf}}%
  \subfigure[Accuracy under different FLOPS]{\includegraphics[width=0.5\linewidth]{img/bert_acc_flops.pdf}}
  \caption{The accuracy of Bert models on the MNLI dataset.}
    \label{img:img-dimension}
\end{figure*}

% \begin{figure*}[htbp]
%     \centering
%   \subfigure[Test accuracy using various numbers of attention heads on Bert]{\includegraphics[width=0.5\linewidth]{img/mt-dnn.png}}%
%     \label{img:bert}
% \end{figure*}

% \subsubsection{Principles for masking neurons in different layers}
% \begin{align*}
%     \max\limits_{x,y,z\in \mathbb{N}} \quad &\ell_{val}(x,y,z)\\
%     \textrm{s.t.} \quad & ax+by+cz \le D
% \end{align*}+
% \yx{greedy coordinate descent?}
% \begin{proposition}
% Assume the input $x \sim \gN(0,I) \in \mathbb{R}^D$, and in layer $l$ the parameters $W_l \sim \gN(0,I) \in \mathbb{R}^{k_{l-1},k_{l}}$. If we randomly mask $d$ neurons in $x$, and denoting the masked input as $\hat{x}$. Then w.h.p, $\Vert (\prod_{i=1}^n W_i)x-(\prod_{i=1}^n W_i)\hat{x}\Vert_2^2=d\prod_{i=1}^n k_l\pm \epsilon$.
% \end{proposition}
% \paragraph{2. Special case (PCA)} If we pick the loss as $l_2$ norm, and the encoder/decoder are constrained to a
% pair of orthogonal matrices up to a transpose, then our method recovers PCA.

% I aim to study the influence of masking neurons in different layers. We treat the masking process as a local perturbation around original neurons. Consider the original nn $f_\theta$ and the masked nn $f_{\hat{\theta}}$. The layer expansion for $f(x)=x\log{x/y}\approx (x-y) + \frac{(x-y)^2}{2y}$. Then the KL-divergence between the two NNs is
% \begin{align*}
%     \E_x\left[D_{KL}(f_\theta(x) || f_{\hat{\theta}}(x))\right]&= \E_x\left[\sum_i f_\theta(x)_i\log{f_\theta(x)_i/f_{\hat{\theta}}(x)_i}\right]\\
%     &\approx\E_x\left[\sum_i f_\theta(x)_i-f_{\hat{\theta}}(x)_i + (f_\theta(x)_i-f_{\hat{\theta}}(x)_i)^2 /f_{\hat{\theta}}(x)_i \right]\\
%     &=\E_x\left[\sum_i (f_\theta(x)_i-f_{\hat{\theta}}(x)_i)^2 /f_{\hat{\theta}}(x)_i \right]
% \end{align*}

% \subsubsection{Convergence analysis} Easy to prove by keeping track of the training dynamics of NTK. 


% \paragraph{Remark:Does the ordering make optimization more easier?}

% - Assume the reduction on the accuracy decreases when we continually add neurons. 

% - Shall take the task structure explicitly. What setting the framework can boost accuracy? 

% - loss landscape: empirical shows that the loss landscape neurons $i$ in two cases:
% (i) conventional CNN, only change the parameters in the $i$-th neurons.
% (ii) ordered neuron, when masking out $>i$-th neurons.

\subsection{Relationship to boosting}

Boosting trains classifiers one by one, and it will \textbf{not} adapt previous classifiers when training later ones. In contrast, in ordered neurons, all channels can \textbf{adapt together}. It would make optimization more easier for the latter ones.

% \paragraph{1. Convergence analysis for boosting on neural network}:

% Follow \cite{Mason1999BoostingAA}, we can regard boosting as gradient descent on the function space. More specifically, we would like to find a weak classifier $\theta_i$ such that 
% \begin{align*}
%     \theta_i &= \argmin_{\theta}\langle \nabla \Ls(f_{\theta_1,\dots,\theta_{i-1}}), f_{\theta} \rangle\\
%     &=\argmin_{\theta} \sum\limits_{j=1}^m \frac{\nabla f_{\theta_1,\dots,\theta_{i-1}}(x_j)_{y_j}}{f_{\theta_1,\dots,\theta_{i-1}}(x_j)_{y_j}}f_{\theta}(x_j)_{y_j}
% \end{align*}
% \textbf{Remark}. It's easy to prove its convergence. If we further constraint the space of $\theta$ to be the convex hull of a set of fixed neurons $\gM$. $\theta = \argmin_{\theta \in \gM}\langle \nabla \Ls(f_{\theta_1,\dots,\theta_{i-1}}), f_{\theta} \rangle$, then it's exactly the method used in \cite{Ye2020GoodSP}, which greedily selects the neuron that minimizes the loss function (their convergence follows the analysis of Frank-Wolfe algorithm).

% \paragraph{2. Boosting cannot adapt together, while order neurons can:}

% The example is shown in \figref{fig:my_label}. 
% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{img/example.png}
%     \caption{The first classifier $f_1$ can adapt to improve the accuracy}
%     \label{fig:my_label}
% \end{figure}

\subsection{Applications}

Some potential applications:

1. Test time computational capacity versus test accuracy trade-off

2. Uncertainty calibration (https://arxiv.org/pdf/2006.08437.pdf)

3. Robust to label noise/OOD generalization, OOD detection /adversarial certification radius, robustness
% % Consider the loss function $C(f)$. Basically boosting optimize it by gradient descent on the function space
% % \begin{align*}
% %     f_1^* = \argmin_{f}C(f), f_2^* = \argmin_{f_2}C(f_1^*+\epsilon f_2)
% % \end{align*}

% % Instead, the order neurons have the following objection:
% % \begin{align*}
% %     f_1^o,f_2^o = C(f_1)+C(f_1+\epsilon f_2)
% % \end{align*}

% % Some basic results:
% % \begin{enumerate}
% %     \item $C(f_1^*)+C(f_1^*+\epsilon f_2^*) \ge C(f_1^o)+C(f_1^o+\epsilon f_2^o)$
% % \end{enumerate}
% % \section{Auxiliary task selection}

% % \subsection{Experiment}

% % \begin{figure*}[htbp]
% %     \centering
% %   \subfigure[Test accuracy using various number of channels ]{\includegraphics[width=0.5\linewidth]{img/acc_index.pdf}}%
% %   \subfigure[Reduction of Accuracy w.r.t the channel index]{\includegraphics[width=0.5\linewidth]{img/acc_index_diff_3.pdf}}
% %     \label{img:img-dimension}
% % \end{figure*}

\bibliographystyle{unsrt}
\bibliography{bib}

\appendix

\section{Proof for theorems}
\begin{proof}
\label{proof}
For simplicity we denote the distribution of the stochastic part (first $i$ channels)  as $q_{\theta}(z_{\le i}|x)$, and similarly we denote the output of classifier as $p_{\phi}(y|z_{\le i})$. We first reformulate the objective 
\begin{align}
    \mathcal{L} &= -\mathbb{E}_{x,y \sim p_d(x,y), i \sim \mathcal{U}\{1, K\}}\mathbb{E}_{z \sim q_{\theta}(z_{\le i}|x)}[\log p_{\phi}(y|z_{\le i})]\nonumber\\
    & = \frac{-1}{K}\sum_{i=1}^K \mathbb{E}_{x,y \sim p_d(x,y)}\mathbb{E}_{z \sim q_{\theta}(z_{\le i}|x)}[\log p_{\phi}(y|z_{\le i})]\nonumber\\
    &= \frac{-1}{K}\sum_{i=1}^K \int q_{\theta}(z_{\le i},y)\log p_{\phi}(y|z_{\le i}) dy dz_{\le i} \qquad\qquad (p_d(y)q_{\theta}(z_{\le i}|y) =q_{\theta}(z_{\le i},y)) \nonumber\\
    &\ge \frac{-1}{K}\sum_{i=1}^K \int q_{\theta}(z_{\le i},y)\log q_{{\theta}}(y|z_{\le i}) dy dz_{\le i} \label{ieq:KL-term}
\end{align}

The inequality~(\ref{ieq:KL-term}) holds because KL-divergences are non-negative. %The equality holds when $q_{\theta}(y|z_{\le i}) = p_{\phi}(y|z_{\le i})$.  
Under the assumption of an optimal classifier $\phi$, we can achieve the equality in (\ref{ieq:KL-term}), in which case the objective equals
\begin{align}
     \mathcal{L}  &= \frac{-1}{K}\sum_{i=1}^K \int q_{\theta}(z_{\le i},y)\log \frac{q_{\theta}(y,z_{\le i})}{q_{\theta}(z_{\le i})} dy dz_{\le i} \nonumber
\end{align}
We can define the following modified objective by adding the label entropy term, since it is a constant independent of $\theta$.
\begin{align}
    \mathcal{L} &= \frac{-1}{K}\sum_{i=1}^K \int q_{\theta}(z_{\le i},y)\log \frac{q_{\theta}(y,z_{\le i})}{q_{\theta}(z_{\le i})p_d(y)} dy dz_{\le i} \nonumber \\
    &= \frac{-1}{K}\sum_{i=1}^K I(y;z_{\le i})\label{eq:mutual-sum}
\end{align}

If there exists an integer $i \in \{2,\cdots, K\}$ such that $I(z_i;y|z_{\le i-1}) > I(z_{i-1};y|z_{\le i-2})$, we can exchange the position of $z_i$ and $z_{i-1}$ to increase the value of objective~(\ref{eq:mutual-sum}). By the chain rule of mutual information we have:
\begin{align}
&I(y;z_{i},z_{i-1},z_{\le i-2}) = I(z_{i-1},z_{\le i-2};y) + I(z_{i};y|z_{\le i-1})\nonumber\\
&=I(z_{i},z_{\le i-2};y) + I(z_{i-1};y|z_{\le i-2},z_i).\nonumber
\end{align}
When $I(z_i;y|z_{\le i-1}) > I(z_{i-1};y|z_{\le i-2})$, we can show that $I(y;z_{i},z_{\le i-2}) > I(y;z_{i-1},z_{\le i-2})$:
\begin{align}
    &I(y;z_{i},z_{\le i-2}) - I(y;z_{i-1},z_{\le i-2})\nonumber\\
    &= I(z_{i};y|z_{\le i-1}) - I(z_{i-1};y|z_{\le i-2},z_i)\nonumber\\
    &> I(z_{i-1};y|z_{\le i-2}) - I(z_{i-1};y|z_{\le i-2},z_i)\nonumber \\
    &= I(y,z_{i};z_{i-1}|z_{\le i-2})- I(y;z_{i-1}| z_{\le i-2},z_i)\label{ineq:z-ind}\\
    &= I(z_i;z_{i-1}|z_{\le i-2}) \ge 0,
\end{align}
where \eqref{ineq:z-ind} holds by the chain rule of mutual information: $I(z_{i-1};y|z_{\le i-2})=I(y,z_{i};z_{i-1}|z_{\le i-2}) - I(z_i;z_{i-1}|y,z_{\le i-2})$, and $I(z_i;z_{i-1}|y,z_{\le i-2})=0$ by the conditional independence assumption $z_i \perp z_{i-1}|y,z_{\le i-2}$. Hence if we exchange the position of $z_i$ and $z_{i-1}$ of the latent vector $z$, we can show that the new objective value after the position switch is strictly smaller than the original one:
\begin{align}
    &\frac{-1}{K}\left(\sum_{k=1}^{i-2} I(y;z_{\le k}) + I(y;z_{\le i-2},z_i)+ \sum_{k=i}^{K} I(y;z_{\le i})\right)\nonumber\\
    &< \frac{-1}{K}\left(\sum_{k=1}^{i-2} I(y;z_{\le k}) + I(y;z_{\le i-2},z_{i-1})+\sum_{k=i}^{K} I(y;z_{\le i})\right)\label{ineq:switch}\\
    &= \frac{-1}{K}\sum_{k=1}^K I(y;z_{\le k}).\nonumber
\end{align}

Inequality~(\ref{ineq:switch}) holds by $I(y;z_{i},z_{\le i-2})> I(y;z_{i-1},z_{\le i-2})$. From above we can conclude that if the encoder is optimal, then the following inequalities must hold:
$$\forall i \in \{2,\cdots, K\}:~~ I(z_i;y | z_{\le i-1}) \le I(z_{i-1};y | z_{\le i-2}).$$
Otherwise we can exchange the dimensions to make the objective \eqnref{eq:mutual-sum} smaller, which contradicts the optimally of encoder $\theta$.
\end{proof}
